Image Smoothing via Unsupervised Learning

Image smoothing represents a fundamental component of many disparate computer vision and graphics applications. In this paper, we present a unified unsupervised (label-free) learning framework that facilitates generating flexible and high-quality smoothing effects by directly learning from data using deep convolutional neural networks (CNNs). The heart of the design is the training signal as a novel energy function that includes an edge-preserving regularizer which helps maintain important yet potentially vulnerable image structures, and a spatially-adaptive Lp flattening criterion which imposes different forms of regularization onto different image regions for better smoothing quality. We implement a diverse set of image smoothing solutions employing the unified framework targeting various applications such as, image abstraction, pencil sketching, detail enhancement, texture removal and content-aware image manipulation, and obtain results comparable with or better than previous methods. Moreover, our method is extremely fast with a modern GPU (e.g, 200 fps for 1280x720 images). Our codes and model are released in https://github.com/fqnchina/ImageSmoothing.

==> fig-blur1.tex <==
\setlength{\tabcolsep}{1pt}
\begin{figure}[htp]
\begin{center}
\begin{tabular}{ccc}

\includegraphics[width=2.8cm]{demo12-500-7-input.jpg}
&\includegraphics[width=2.8cm]{demo12-500-7-input-predict_standard_blur_L2_weight5_window0_threshold_20_10_window2_L08_w0_epoch30.jpg}
&\includegraphics[width=2.8cm]{demo12-500-7-input-predict_standard_saliency_sharpen_L2_weight5_window0_threshold_20_10_window1_L08_w0_epoch30-detail.jpg}
\\

\includegraphics[width=2.8cm]{demo12-500-9-input.jpg}
&\includegraphics[width=2.8cm]{demo12-500-9-input-predict_standard_blur_L2_weight5_window0_threshold_20_10_window2_L08_w0_epoch30.jpg}
&\includegraphics[width=2.8cm]{demo12-500-9-input-predict_standard_saliency_sharpen_L2_weight5_window0_threshold_20_10_window1_L08_w0_epoch30-detail.jpg}
\\

\includegraphics[width=2.8cm]{demo11-500-22-input.jpg}
&\includegraphics[width=2.8cm]{demo11-500-22-input-predict_standard_blur_L2_weight5_window0_threshold_20_10_window2_L08_w0_epoch30.jpg}
&\includegraphics[width=2.8cm]{demo11-500-22-input-predict_standard_saliency_sharpen_L2_weight5_window0_threshold_20_10_window1_L08_w0_epoch30-detail.jpg}
\\
%\includegraphics[width=2.8cm]{smooth2-7-input.jpg}
%%&\includegraphics[width=2.8cm]{smooth2-7-input-predict_standard_blur_L2_weight3_window0_threshold_20_10_epoch30.jpg}
%&\includegraphics[width=2.8cm]{smooth2-7-input-predict_standard_blur_L2_weight5_window0_threshold_20_10_window2_L08_w1_epoch30.jpg}
%&\includegraphics[width=2.8cm]{smooth2-7-input-predict_standard_blur_L2_weight5_window0_threshold_20_10_window2_L08_w1_epoch30_sharpen-1.jpg}
%\\
%
%\includegraphics[width=2.8cm]{demo2-new-6.jpg}
%%&\includegraphics[width=2.8cm]{demo2-new-6-predict_standard_blur_L2_weight3_window0_threshold_20_10_epoch30.jpg}
%&\includegraphics[width=2.8cm]{demo2-new-6-predict_standard_blur_L2_weight5_window0_threshold_20_10_window2_L08_w1_epoch30.jpg}
%&\includegraphics[width=2.8cm]{demo2-new-6-predict_standard_blur_L2_weight5_window0_threshold_20_10_window2_L08_w1_epoch30_sharpen-1.jpg}
%\\
%
%\includegraphics[width=2.8cm]{demo-new2-2.jpg}
%%&\includegraphics[width=2.8cm]{demo-new2-2-predict_standard_blur_L2_weight3_window0_threshold_20_10_epoch30.jpg}
%&\includegraphics[width=2.8cm]{demo-new2-2-predict_standard_blur_L2_weight5_window0_threshold_20_10_window2_L08_w1_epoch30.jpg}
%&\includegraphics[width=2.8cm]{demo-new2-2-predict_standard_blur_L2_weight5_window0_threshold_20_10_window2_L08_w1_epoch30_sharpen-1.jpg}
%\\

%\includegraphics[width=2.8cm]{smooth2-147-input.jpg}
%%&\includegraphics[width=2.8cm]{smooth2-147-input-predict_standard_blur_L2_weight3_window0_threshold_20_10_epoch30.jpg}
%&\includegraphics[width=2.8cm]{smooth2-147-input-predict_standard_blur_L2_weight5_window0_threshold_20_10_window2_L08_w1_epoch30.jpg}
%\\

%\includegraphics[width=2.8cm]{demo2-new-8.jpg}
%%&\includegraphics[width=2.8cm]{smooth2-147-input-predict_standard_blur_L2_weight3_window0_threshold_20_10_epoch30.jpg}
%&\includegraphics[width=2.8cm]{demo2-new-8-predict_standard_blur_L2_weight5_window0_threshold_20_10_window2_L08_w1_epoch30.jpg}
%&\includegraphics[width=2.8cm]{demo2-new-8-predict_standard_blur_L2_weight5_window0_threshold_20_10_window2_L08_w1_epoch30_sharpen-1.jpg}
%\\
\small{Input} & \small{Background smoothed} & \small{Foreground enhanced}
\\

\end{tabular}
\end{center}
\vspace{-3mm}
\caption{Content-aware image manipulation with our method.}
\label{figure:background1}
\end{figure}


==> fig-blur2.tex <==
\setlength{\tabcolsep}{1pt}
\begin{figure}[htp]
\begin{center}
\begin{tabular}{ccc}

\includegraphics[width=2.8cm]{demo12-500-25-input.jpg}
&\includegraphics[width=2.8cm]{demo12-500-25-input-predict_standard_blur_L2_weight5_window0_threshold_20_10_window2_L08_w0_epoch30.jpg}
&\includegraphics[width=2.8cm]{demo12-500-25-input-predict_standard_saliency_sharpen_L2_weight5_window0_threshold_20_10_window1_L08_w0_epoch30-detail.jpg}
\\

\includegraphics[width=2.8cm]{demo11-500-13-input.jpg}
&\includegraphics[width=2.8cm]{demo11-500-13-input-predict_standard_blur_L2_weight5_window0_threshold_20_10_window2_L08_w0_epoch30.jpg}
&\includegraphics[width=2.8cm]{demo11-500-13-input-predict_standard_saliency_sharpen_L2_weight5_window0_threshold_20_10_window1_L08_w0_epoch30-detail.jpg}
\\

%\includegraphics[width=2.8cm,trim={0 2cm 0 1.5cm},clip]{smooth2-112-input.jpg}
%%&\includegraphics[width=2.8cm,trim={0 2cm 0 1.5cm},clip]{smooth2-112-input-predict_standard_blur_L2_weight3_window0_threshold_20_10_epoch30.jpg}
%&\includegraphics[width=2.8cm,trim={0 2cm 0 1.5cm},clip]{smooth2-112-input-predict_standard_blur_L2_weight5_window0_threshold_20_10_window2_L08_w1_epoch30.jpg}
%&\includegraphics[width=2.8cm,trim={0 2cm 0 1.5cm},clip]{smooth2-112-input-predict_standard_blur_L2_weight5_window0_threshold_20_10_window2_L08_w1_epoch30_sharpen-1.jpg}
%\\
%
%\includegraphics[width=2.8cm]{demo-new2-2.jpg}
%%&\includegraphics[width=2.8cm]{demo-new2-2-predict_standard_blur_L2_weight3_window0_threshold_20_10_epoch30.jpg}
%&\includegraphics[width=2.8cm]{demo-new2-2-predict_standard_blur_L2_weight5_window0_threshold_20_10_window2_L08_w1_epoch30.jpg}
%&\includegraphics[width=2.8cm]{demo-new2-2-predict_standard_blur_L2_weight5_window0_threshold_20_10_window2_L08_w1_epoch30_sharpen-1.jpg}
%\\
\small{Input} & \small{Background smoothed} & \small{Foreground enhanced}
\\
\end{tabular}
\end{center}
\vspace{-3mm}
\caption{Content-aware image manipulation with our method.}
\label{figure:background2}
\end{figure}


==> fig-compSelf-edge.tex <==
\setlength{\tabcolsep}{1pt}
\begin{figure*}[htp]
\begin{center}
\begin{tabular}{ccccc}

%\includegraphics[width=3.5cm,trim={0 1.5cm 0 5.9cm},clip]{demo-5.jpg}
%&\includegraphics[width=3.5cm,trim={0 1.5cm 0 5.9cm},clip]{demo-5-predict_standard_selfcomp_edgePreserving_L2_weight3_window4_threshold_20_10_woEdge_epoch24.jpg}
%&\includegraphics[width=3.5cm,trim={0 1.5cm 0 5.9cm},clip]{demo-5-predict_standard_edgePreserving_L2_weight3_window4_threshold_20_10_same_epoch30.jpg}
%&\includegraphics[width=3.5cm,trim={0 1.5cm 0 5.9cm},clip]{demo-5-input-edge.jpg}
%&\includegraphics[width=3.5cm,trim={0 1.5cm 0 5.9cm},clip]{demo-5-edge.jpg}
%\\

%\includegraphics[width=3.5cm,trim={0 0.7cm 0 0},clip]{smooth-63-input.jpg}
%%&\includegraphics[width=3.5cm,trim={0 0 0 0},clip]{smooth-63-input-predict_standard_selfcomp_edgePreserving_L2_weight3_window4_threshold_20_10_woEdge_epoch24.jpg}
%%&\includegraphics[width=3.5cm,trim={0 0 0 0},clip]{smooth-63-input-predict_standard_edgePreserving_L2_weight3_window4_threshold_20_10_same_epoch30.jpg}
%&\includegraphics[width=3.5cm,trim={0 0.7cm 0 0},clip]{smooth-63-input-predict_standard_selfcomp_edgePreserving_L2_weight5_window3_threshold_20_10_window10_L08_w1_woEdge_epoch30.jpg}
%&\includegraphics[width=3.5cm,trim={0 0.7cm 0 0},clip]{smooth-63-input-predict_standard_edgePreserving_L2_weight5_window3_threshold_20_10_window10_L08_w1_epoch30.jpg}
%&\includegraphics[width=3.5cm,trim={0 0.7cm 0 0},clip]{smooth-63-input-input-edge.jpg}
%&\includegraphics[width=3.5cm,trim={0 0.7cm 0 0},clip]{smooth-63-input-edge-label.jpg}
%\\

%\includegraphics[width=3.5cm,trim={0 4cm 0 0},clip]{demo9-1-input.jpg}
%&\includegraphics[width=3.5cm,trim={0 4cm 0 0},clip]{demo9-1-input-predict_standard_selfcomp_edgePreserving_L2_weight3_window4_threshold_20_10_woEdge_epoch24.jpg}
%&\includegraphics[width=3.5cm,trim={0 4cm 0 0},clip]{demo9-1-input-predict_standard_edgePreserving_L2_weight3_window4_threshold_20_10_same_epoch30.jpg}
%&\includegraphics[width=3.5cm,trim={0 4cm 0 0},clip]{demo9-1-input-input-edge.jpg}
%&\includegraphics[width=3.5cm,trim={0 4cm 0 0},clip]{demo9-1-input-edge.jpg}
%\\

%\includegraphics[width=3.5cm,trim={0 2cm 0 0},clip]{demo8-500-24-input.jpg}
%&\includegraphics[width=3.5cm,trim={0 2cm 0 0},clip]{demo8-500-24-input-predict_standard_selfcomp_edgePreserving_L2_weight3_window4_threshold_20_10_woEdge_epoch24.jpg}
%&\includegraphics[width=3.5cm,trim={0 2cm 0 0},clip]{demo8-500-24-input-predict_standard_edgePreserving_L2_weight3_window4_threshold_20_10_same_epoch30.jpg}
%&\includegraphics[width=3.5cm,trim={0 2cm 0 0},clip]{demo8-500-24-input-input-edge.jpg}
%&\includegraphics[width=3.5cm,trim={0 2cm 0 0},clip]{demo8-500-24-input-edge.jpg}
%\\

\includegraphics[width=3.5cm,trim={0 0 0 0},clip]{demo9-400-1-input.jpg}
&\includegraphics[width=3.5cm,trim={0 0 0 0},clip]{demo9-400-1-input-predict_standard_selfcomp_edgePreserving_L2_weight5_window3_threshold_20_10_window10_L08_w1_woEdge_epoch30.jpg}
&\includegraphics[width=3.5cm,trim={0 0 0 0},clip]{demo9-400-1-input-predict_standard_edgePreserving_L2_weight5_window3_threshold_20_10_window10_L08_w1_epoch30.jpg}
&\includegraphics[width=3.5cm,trim={0 0 0 0},clip]{demo9-400-1-input-input-edge.jpg}
&\includegraphics[width=3.5cm,trim={0 0 0 0},clip]{demo9-400-1-input-edge.jpg}
\\


%\includegraphics[width=3.5cm,trim={0 0 0 0},clip]{demo9-1-input_vis.jpg}
%&\includegraphics[width=3.5cm,trim={0 0 0 0},clip]{demo9-1-input-predict_standard_selfcomp_edgePreserving_L2_weight5_window3_threshold_20_10_window10_L08_w1_woEdge_epoch30_vis.jpg}
%&\includegraphics[width=3.5cm,trim={0 0 0 0},clip]{demo9-1-input-predict_standard_edgePreserving_L2_weight5_window3_threshold_20_10_window10_L08_w1_epoch30_vis.jpg}
%&\includegraphics[width=3.5cm,trim={0 0 0 0},clip]{demo9-1-input-input-edge.jpg}
%&\includegraphics[width=3.5cm,trim={0 0 0 0},clip]{demo9-1-input-edge.jpg}
%\\


%\includegraphics[width=3.5cm,trim={0 0 0 0},clip]{demo-15_vis.jpg}
%&\includegraphics[width=3.5cm,trim={0 0 0 0},clip]{demo-15-predict_standard_selfcomp_edgePreserving_L2_weight5_window3_threshold_20_10_window10_L08_w1_woEdge_epoch30_vis.jpg}
%&\includegraphics[width=3.5cm,trim={0 0 0 0},clip]{demo-15-predict_standard_edgePreserving_L2_weight5_window3_threshold_20_10_window10_L08_w3_epoch30_vis.jpg}
%&\includegraphics[width=3.5cm,trim={0 0 0 0},clip]{demo-15-input-edge.jpg}
%&\includegraphics[width=3.5cm,trim={0 0 0 0},clip]{demo-15-edge-label.jpg}
%\\
%\includegraphics[width=3.5cm,trim={0 3.5cm 0 0},clip]{demo7-33-input.jpg}
%&\includegraphics[width=3.5cm,trim={0 3.5cm 0 0},clip]{demo7-33-input-predict_standard_selfcomp_edgePreserving_L2_weight3_window4_threshold_20_10_woEdge_epoch24.jpg}
%&\includegraphics[width=3.5cm,trim={0 3.5cm 0 0},clip]{demo7-33-input-predict_standard_edgePreserving_L2_weight3_window4_threshold_20_10_same_epoch30.jpg}
%&\includegraphics[width=3.5cm,trim={0 3.5cm 0 0},clip]{demo7-33-input-input-edge.jpg}
%&\includegraphics[width=3.5cm,trim={0 3.5cm 0 0},clip]{demo7-33-input-edge.jpg}
%\\
%
%\includegraphics[width=3.5cm,trim={0 2cm 1cm 0},clip]{demo10-500-49-input.jpg}
%&\includegraphics[width=3.5cm,trim={0 2cm 1cm 0},clip]{demo10-500-49-input-predict_standard_selfcomp_edgePreserving_L2_weight3_window4_threshold_20_10_woEdge_epoch24.jpg}
%&\includegraphics[width=3.5cm,trim={0 2cm 1cm 0},clip]{demo10-500-49-input-predict_standard_edgePreserving_L2_weight3_window4_threshold_20_10_same_epoch30.jpg}
%&\includegraphics[width=3.5cm,trim={0 2cm 1cm 0},clip]{demo10-500-49-input-input-edge.jpg}
%&\includegraphics[width=3.5cm,trim={0 2cm 1cm 0},clip]{demo10-500-49-input-edge.jpg}
%\\


%\includegraphics[width=3.5cm,trim={0 0cm 0 0},clip]{demo8-500-18-input.jpg}
%&\includegraphics[width=3.5cm,trim={0 0cm 0 0},clip]{demo8-500-18-input-predict_standard_selfcomp_edgePreserving_L2_weight3_window4_threshold_20_10_woEdge_epoch24.jpg}
%&\includegraphics[width=3.5cm,trim={0 0cm 0 0},clip]{demo8-500-18-input-predict_standard_edgePreserving_L2_weight3_window4_threshold_20_10_same_epoch30.jpg}
%&\includegraphics[width=3.5cm,trim={0 0cm 0 0},clip]{demo8-500-18-input-input-edge.jpg}
%&\includegraphics[width=3.5cm,trim={0 0cm 0 0},clip]{demo8-500-18-input-edge.jpg}
%\\

%\includegraphics[width=3.5cm,trim={0 0cm 0 0},clip]{demo8-500-38-input.jpg}
%&\includegraphics[width=3.5cm,trim={0 0cm 0 0},clip]{demo8-500-38-input-predict_standard_selfcomp_edgePreserving_L2_weight3_window4_threshold_20_10_woEdge_epoch24.jpg}
%&\includegraphics[width=3.5cm,trim={0 0cm 0 0},clip]{demo8-500-38-input-predict_standard_edgePreserving_L2_weight3_window4_threshold_20_10_same_epoch30.jpg}
%&\includegraphics[width=3.5cm,trim={0 0cm 0 0},clip]{demo8-500-38-input-input-edge.jpg}
%&\includegraphics[width=3.5cm,trim={0 0cm 0 0},clip]{demo8-500-38-input-edge.jpg}
%\\
Input image & w/o EP criterion & Our result & $E(I)$ & $B$
\\
\end{tabular}
\end{center}
\vspace{-3mm}
\caption{Effectiveness of the proposed edge-preserving (EP) criterion. Trained with the edge-preserving term, our network can better preserve the image structures without sacrificing the flattening effects, and the salient edges kept match well the edges in the binary edge map $B$. Note that $E(I)$ and $B$ were not used to generate the smoothed results (there images are only used in the training stage); we present them here only for reference.}
\label{figure:comp_edge}
\end{figure*}


==> fig-loss-ours.tex <==
\setlength{\tabcolsep}{1pt}
\begin{figure}[t]
\begin{center}
\begin{tabular}{cc}
\includegraphics[width=4.0cm]{train_standard_selfcomp_edgePreserving_L2_weight5_window3_threshold_20_10_window10_L08_w1_woEdge_wo00_calRatio_loss_imgs.jpg}
&\includegraphics[width=4.0cm]{train_standard_selfcomp_edgePreserving_L2_weight5_window3_threshold_20_10_window10_L08_w1_woEdge_wo00_calRatio_ratio_imgs.jpg}
\\
loss & $L_2$ ratio
\\
\end{tabular}
\end{center}
\vspace{-3mm}
\caption{Illustration of the loss curve and $L_2$ ratio curve of the deep learning solver along the training procedure.}
\label{figure:loss_ours}
\vspace{-3mm}
\end{figure}



==> fig-lp_difference.tex <==
\setlength{\tabcolsep}{1pt}
\begin{figure*}[htp]
\begin{center}
\begin{tabular}{ccccccc}
%\includegraphics[width=2.48cm]{demo-15.jpg}
%&\includegraphics[width=2.48cm]{demo-15-predict_standard_selfcomp_edgePreserving_baseline_l2_spatial_epoch30.jpg}
%&\includegraphics[width=2.48cm]{demo-15-predict_standard_selfcomp_edgePreserving_baseline_l2_color_epoch30.jpg}
%&\includegraphics[width=2.48cm]{demo-15-predict_standard_selfcomp_edgePreserving_baseline_l1_color_epoch30.jpg}
%&\includegraphics[width=2.48cm]{demo-15-predict_standard_selfcomp_edgePreserving_baseline_l05_color_epoch30.jpg}
%&\includegraphics[width=2.48cm]{demo-15-predict_standard_selfcomp_edgePreserving_baseline_l01_color_epoch30.jpg}
%\\

%\includegraphics[width=2.48cm]{demo9-400-2-input.jpg}
%&\includegraphics[width=2.48cm]{demo9-400-2-input-predict_standard_selfcomp_edgePreserving_baseline_l2_spatial_epoch30.jpg}
%&\includegraphics[width=2.48cm]{demo9-400-2-input-predict_standard_selfcomp_edgePreserving_baseline_l2_color_epoch30.jpg}
%&\includegraphics[width=2.48cm]{demo9-400-2-input-predict_standard_selfcomp_edgePreserving_baseline_l1_color_epoch30.jpg}
%&\includegraphics[width=2.48cm]{demo9-400-2-input-predict_standard_selfcomp_edgePreserving_baseline_l08_color_epoch30.jpg}
%&\includegraphics[width=2.48cm]{demo9-400-2-input-predict_standard_selfcomp_edgePreserving_baseline_l05_color_epoch30.jpg}
%&\includegraphics[width=2.48cm]{demo9-400-2-input-predict_standard_selfcomp_edgePreserving_baseline_l01_color_epoch30.jpg}
%\\

\includegraphics[width=2.48cm]{demo9-400-2-input-line.jpg}
&\includegraphics[width=2.48cm]{demo9-400-2-input-IRLS-L01_15-20-small-new.jpg}
&\includegraphics[width=2.48cm]{demo9-400-2-input-IRLS-L05_15-20-small-new.jpg}
&\includegraphics[width=2.48cm]{demo9-400-2-input-IRLS-L08_15-20-small-new.jpg}
&\includegraphics[width=2.48cm]{demo9-400-2-input-IRLS-L1_1-20-small-new.jpg}
&\includegraphics[width=2.48cm]{demo9-400-2-input-IRLS-L2_1-1-small-new.jpg}
&\includegraphics[width=2.48cm]{demo9-400-2-input-IRLS-L2_01_spatial-1-small-new.jpg}
\\

\includegraphics[width=2.48cm]{fig-demo9-400-2-input.jpg}
&\includegraphics[width=2.48cm]{fig-demo9-400-2-input-IRLS-L01_15-20-small-new.jpg}
&\includegraphics[width=2.48cm]{fig-demo9-400-2-input-IRLS-L05_15-20-small-new.jpg}
&\includegraphics[width=2.48cm]{fig-demo9-400-2-input-IRLS-L08_15-20-small-new.jpg}
&\includegraphics[width=2.48cm]{fig-demo9-400-2-input-IRLS-L1_1-20-small-new.jpg}
&\includegraphics[width=2.48cm]{fig-demo9-400-2-input-IRLS-L2_1-1-small-new.jpg}
&\includegraphics[width=2.48cm]{fig-demo9-400-2-input-IRLS-L2_01_spatial-1-small-new.jpg}
\\

%\includegraphics[width=2.48cm]{fig-demo9-400-2-input.jpg}
%&\includegraphics[width=2.48cm]{fig-demo9-400-2-input-predict_standard_selfcomp_edgePreserving_baseline_l2_spatial_epoch30-2.jpg}
%&\includegraphics[width=2.48cm]{fig-demo9-400-2-input-predict_standard_selfcomp_edgePreserving_baseline_l2_color_epoch30-2.jpg}
%&\includegraphics[width=2.48cm]{fig-demo9-400-2-input-predict_standard_selfcomp_edgePreserving_baseline_l1_color_epoch30-2.jpg}
%&\includegraphics[width=2.48cm]{fig-demo9-400-2-input-predict_standard_selfcomp_edgePreserving_baseline_l08_color_epoch30-2.jpg}
%&\includegraphics[width=2.48cm]{fig-demo9-400-2-input-predict_standard_selfcomp_edgePreserving_baseline_l05_color_epoch30-2.jpg}
%&\includegraphics[width=2.48cm]{fig-demo9-400-2-input-predict_standard_selfcomp_edgePreserving_baseline_l01_color_epoch30-2.jpg}
%\\

%\includegraphics[width=2.48cm]{demo9-600-5-input.jpg}
%&\includegraphics[width=2.48cm]{demo9-600-5-input-predict_standard_selfcomp_edgePreserving_baseline_l2_spatial_epoch30.jpg}
%&\includegraphics[width=2.48cm]{demo9-600-5-input-predict_standard_selfcomp_edgePreserving_baseline_l2_color_epoch30.jpg}
%&\includegraphics[width=2.48cm]{demo9-600-5-input-predict_standard_selfcomp_edgePreserving_baseline_l1_color_epoch30.jpg}
%&\includegraphics[width=2.48cm]{demo9-600-5-input-predict_standard_selfcomp_edgePreserving_baseline_l05_color_epoch30.jpg}
%&\includegraphics[width=2.48cm]{demo9-600-5-input-predict_standard_selfcomp_edgePreserving_baseline_l01_color_epoch30.jpg}
%\\
Input &  $L_{0.1}$  & $L_{0.5}$ & $L_{0.8}$ & $L_{1}$ & $L_2$ & $L_2$ $(w^s)$
\end{tabular}
\end{center}
\vspace{-3mm}
\caption{Image smoothing results with different $L_p$ regularization in the smoothness term. Gaussian weights with color affinity is used for these results except for the last one which uses spatial affinity. The bottom row show the resultant brightness values on the 1D image slice indicated by the red line. Smaller $p$ values can well flatten the details and preserve the important structures, but spurious edges may arise (known as the staircasing artifact). A large $p$ value such as $p=2$ may lead to blurry results and miss some important image structures.}
\label{figure:Lp_comparison}
\vspace{-3mm}
\end{figure*}
% Zoom in three different regions in the bottom of the image


==> fig-teaser.tex <==
\setlength{\tabcolsep}{1pt}
\begin{figure*}[t]
\begin{center}
\begin{tabular}{cccccc}
Input & BLF & WLS & $L_0$ & FGS & Ours
\\

\includegraphics[width=2.8cm]{flower-20-input.jpg}
&\includegraphics[width=2.8cm]{flower-20-BLF.jpg}
&\includegraphics[width=2.8cm]{flower-20-WLS.jpg}
&\includegraphics[width=2.8cm]{flower-20-L0smooth.jpg}
&\includegraphics[width=2.8cm]{flower-20-FGS.jpg}
&\includegraphics[width=2.8cm]{flower-20-input-predict_edgeMaintain_Diminish_3_l2_3_w20_lt03_Preserve_n12_01_W1_new_e15.jpg}
%&\includegraphics[width=2.8cm]{flower-20-input-predict_EdgePreserving_W4_win_7_30.jpg}
\\

\includegraphics[width=2.8cm]{flower-20-input.jpg}
&\includegraphics[width=2.8cm]{flower-20-BLF-detail.jpg}
&\includegraphics[width=2.8cm]{flower-20-WLS-detail.jpg}
&\includegraphics[width=2.8cm]{flower-20-L0smooth-detail.jpg}
&\includegraphics[width=2.8cm]{flower-20-FGS-detail.jpg}
&\includegraphics[width=2.8cm]{flower-20-input-predict_edgeMaintain_Diminish_3_l2_3_w20_lt03_Preserve_n12_01_W1_new_e15-detail.jpg}
%&\includegraphics[width=2.8cm]{flower-20-input-predict_EdgePreserving_W4_win_7_30-detail.jpg}
\\

\end{tabular}
\end{center}
\vspace{-3mm}
\caption{Detail Magnification.}
\label{figure:detail}
\end{figure*}


==> introduction.tex <==
\section{Introduction}

The goal of image smoothing is to eliminate unimportant fine-scale details while maintaining primary image structures. This technique has been applied to a wide range of computer vision and graphics applications, each of which demands a unique design of an image smoothing algorithm. For the example of detail enhancement, \cite{WLS} is developed to construct an edge-preserving image decomposition of a residual detail layer and a smooth base layer, which is prevented from being over sharpened, otherwise the gradient reversal artifact is very likely to appear in the exaggerated image. As for image abstraction and pencil sketching, \cite{L0smooth} is designed to smooth out the moderate gradient regions while preserving and enhancing the salient sharp edges, which are extracted further for these stylization effects. However, the enhanced image structure in the smooth image tends to produce the aforementioned artifacts in the detail enhancement application. Some recent work \cite{RTV,RGF} are devoted to maintain the meaningful image structures while removing the distractive repetitive small-scale textures, where color transition could still be significant, which will be probably maintained by the previous image smoothing approaches \cite{WLS,L0smooth}.

The complexity of independent design for distinct applications is unintelligible and non user-friendly. Therefore, the question we explore is if there is a unified framework to integrate the different image smoothing effects with only subtle modifications to the system. We observe that the core and main difference for these image smoothing algorithms is to determine which part of image structure to depress (image smoothing) and which part of them to preserve or even enhance (edge-preserving), for instance, \cite{RTV} eliminates the fine-scale high-contrast textures, and \cite{L0smooth} removes only the low-amplitude details and maintains salient structures.

Therefore, to address such a problem, we propose two novel measures for optimization, 1) the spatially adaptive $L_p$ flattening criterion and 2) the edge-preserving criterion. The key idea for the first measure is that we employ different sparsity-inducing regularization known as $L_p$ norm that characterises distinct smoothing effects, and allocate them differently in the spatial domain in accordance to a guidance edge map. This is drastically different from many previous work which utilizes single $L_p$ norm over the whole image. By doing so, our algorithm benefits from not only overcoming the side-effects caused by an individual regularization, such as staircasing artifacts produced by small $L_p$ norm ($0<p<1$), but also enables the implementation of multiple different smoothing effects thanks to various regularization spatially specified by the guidance edge map. Note the edge preservation task is implicitly embedded in the flattening criterion by setting a reasonable small standard deviation of Gaussian weight for the $L_p$ norm like the previous approaches. To preserve the important image structures in a more direct and effective manner, our second criterion explicitly highlights them by minimizing the quadratic difference between the computed edge map from predicted smooth image and the required edge map from the input image, which is determined by some basic principles and labeled by users both.

Deep learning has been successfully applied in directly learning the desired supervised target in an end-to-end manner for many computer vision and graphics tasks, e.g. object detection, segmentation, image super-resolution, reflection removal, etc. However, deep learning has been barely utilized as a solution to the optimization problem without ground truth labels for supervised training.

In this paper, we treat deep learning as a numerical solver to optimize an objective function in an weakly-supervised way. The proposed objective function is implemented as a loss layer with back propagation which enables gradient descent in optimizing the deep neural network. In the learning stage, we train a deep network to iteratively minimize the objective function, and feed a new image through the network without the need of optimizing the objective function again in the evaluation stage.

The deep learning solver makes a big difference from traditional optimization methods in mainly three sides, 1). The classical optimization process is usually computationally expensive and time consuming for many iterative minimizations. The deep learning solver is presented as a deep neural network, which requires only one feed forward pass for evaluation and is therefore usually very efficient. 2). An effective trivial solution to a sophisticated objective function is difficult to be resolved in many cases, while the restriction to a deep learning solution is very limited: as long as the objective function is differentiable to the optimized target, it can be trivially optimized by the deep network, which is very easy to implement. 3). Except for input image, extra inputs like guidance image in our proposed measures is no longer required in the evaluation stage, which is not the case for the traditional methods.

All in all, the contribution of this paper lies as follows,
\begin{itemize}
\item We introduce a novel image smoothing objective function, built on the mixture of a spatially adaptive $L_p$ flattening criterion and an edge-preserving criterion. By minimizing the proposed criterions, our algorithm is able to achieve state-of-the-art image smoothing effects.
\item We are able to implement multiple different image smoothing effects within a single framework. The only variable responsible for the distinct smoothing effects is the guidance edge map, which can be detected based on some basic principles and modified by user further.
\item We propose a new deep learning based solution pipeline to the aforementioned image smoothing criterion. The optimization process is learned into the deep network which is represented as an end-to-end mapping for evaluation. The proposed solver runs much faster than most traditional image smoothing algorithms.
\end{itemize}



%*******************second version**********************
%Image smoothing is an essential tool to implement multiple different image processing and computer graphics applications. For example, edge preserving smoothing is required to generate some stylization effects like image abstraction, pencil sketching, \emph{etc}. By extracting the detail layer from the input and edge-preserving smoothing image, the subtle image details can be enhanced for better visualization. Specialized smoothing measure \cite{RTV} and framework \cite{RGF} are developed to remove the small-scale textures while maintaining the visually important image structures. More recently, the bokeh effects generated by the large aperture with professional lens has been approximated on the smart phones. Some famous app like Snapseed and smart phone producers like Huawei and Oppo have implemented similar functions to enable beautiful background blur effects. All the different applications demand specific and distinct design of the algorithm, for example, texture removal requires to eliminate the distractive repetitive small-scale structures where color transition may be even significant, however edge-preserving smoothing will maintain such edges.
%
%Various different smoothing effects can be implemented by minimizing the flattening criterion equipped with distinct $L_p$ norm. For example, $L_p$ norm (0<p<1) performs very well in achieving strong smoothing effects, but tends to create staircasing artifacts within moderate smooth regions by breaking them up into piecewise constant regions separated by spurious edges, while $L_p$ norm (p=2) is able to generate blurry images and wipe out the edges.
%
%To implement all the drastically different smoothing effects within a single framework, we propose a spatially variant $L_p$ norm flattening criterion, which applies $L_{0.5}$ and $L_2$ norm in distinct image regions in accordance to a user specified edge map. For the example of edge-preserving image smoothing, $L_{0.5}$ norm is utilized among the whole image except for the over-sharpened patchy regions, which are covered by $L_2$ norm to blur the spurious edges.
%
%As $L_{0.5}$ norm is employed, the smooth image becomes sharp, and the edges with conspicuous color transition are easily maintained well. By minimizing the flattening criterion, the nearby pixels with similar colors tends to be put even closer. Some slender edges whose two sides share similar color values tend to be over smoothed, but they still could be semantically important. To overcome the challenges, we present an edge-preserving criterion to explicitly highlight the desired valuable structures guided by the same edge map utilized in the flattening criterion.
%
%To transform between different smoothing applications within the same framework, we only need to adjust the feeded edge map which indicates various smoothing effects in distinct regions.
%
%Instead of exploiting traditional numerical solver to optimize the objective function, in this paper, we propose to employ an efficient fully-convolutional deep neural network which learns to minimize the proposed criterions. Note the benefits of our deep learning based solver lies in three aspects. \emph{(a)}, the deep network is learned as an end-to-end mapping which characterizes the smoothing effects. It requires only the input image for evaluation since the guided edge map is incorporated into the criterions for only training. \emph{(b)}, our deep learning based solver runs much faster than the other optimization based smoothing strategies, as only one forward pass is needed for testing instead of multiple iterations in traditional methods. \emph{(c)}, deep learning provides a new pathway to optimize the objective functions which are too complex to find an efficient and effective traditional solver. The details of optimization process is represented in the deep network.
%
%All in all, the contribution of this paper lies as follows,
%\begin{itemize}
%\item We introduce a new image smoothing measure, built on the mixture of a spatially adaptive $L_p$ norm flattening criterion and an edge-preserving criterion guided by the same edge map. By minimizing the proposed criterions, our algorithm is able to achieve state-of-the-art various different image smoothing effects.
%\item We are the first to implement multiple different image smoothing effects within a single framework, such as edge-preserving smoothing, texture removal, background blur out of saliency, \emph{etc}. The only variable responsible for the distinct smoothing effects is the edge map, which can be detected or even user designed.
%\item We propose a new deep learning based solution pipeline to the above image smoothing criterion. The optimization process is learned into the deep network which is represented as an end-to-end mapping for evaluation. The proposed solver is very efficient and doesn't require the guided edge map in the test stage.
%\end{itemize}
%*******************second version**********************




%*******************first version**********************
%Various degrees of details and structures are filled in natural images. To perform a better manipulation and understanding of the scene, it is crucial to extract the sparse salient structures and diminish the insignificant details in accordance with human visual perception, which is exactly the goal of edge-preserving image smoothing. The generality and effectiveness of this technique is exemplified in many image processing and computer graphics tasks, like edge extraction, image stylization, pencil sketching, detail enhancement, \emph{etc}.


%Edge aware image smoothing can be achieved by filtering based strategies \cite{anisotropic,BLF98,paris2006fast,weiss2006fast,DT}, which generally calculates the smooth image as a weighted average of the input image. As the above methods are highly restricted to the pixels in the local neighbourhood, the optimization-based approaches \cite{WLS,L0smooth,RTV,FGS,L1smooth} has attracted considerable attention in the last decade, which iteratively seeks a global optimal solution to the objective function which contains a prior flattening term in the sparsity-inducing norm. However, as observed in \cite{L0smooth}, while the smoothing weight becomes larger or the norm becomes smaller, the smooth images tend to be over sharpened and some meaningful edges are diminished by mistake. Moreover, the iterative optimization process is usually complex and time-consuming. Designing a simple and fast solver to the objective function is not easy, either.
%
%To tackle the aforementioned challenges, we propose the hybrid $L_p$/$L_2$ norm based flattening criterion\footnote{In this paper, the constraint ($p < 1$) is defined for $L_p$ norm.}, which not only seeks high-quality smoothness effects with $L_p$ norm, but also overcomes the side effects induced by $L_p$ norm by exploiting $L_2$ norm among the over-sharpened areas. To keep the over-smoothed edges while strong smoothing effect is applied, we present an edge-preserving criterion for explicitly emphasizing these detected thin yet important edges. Since the image structure is maintained well, each separated region becomes even more smoother, and its color is less mixed from the color of other regions.
%
%Unlike previous optimization based smoothing papers, we don't seek an explicit solution to optimize the energy function, but hide the optimization process in an end-to-end mapping learned as a deep neural network, and request only one forward pass given a new natural image, instead of multiple iterations in traditional methods. This is significantly faster than most filtering or optimization based smoothing methods. It treats the detailed solution to the energy function as a black box implemented in the deep neural network. The burden for developing a simple and fast solver is eased from the researchers.
%
%*******************first version**********************

==> introduction_dpw.tex <==
\section{Introduction}

The goal of image smoothing is to eliminate unimportant fine-scale details while maintaining primary image structures. This technique has been applied to a wide range of computer vision and graphics applications, each demanding the unique design of an image smoothing algorithm.

%For example, representative detail magnification tasks involve separating an image into a smooth base layer and a residual detail component, the latter of which can be enhanced and then recombined with the former \cite{WLS}.  In this context the smooth base layer must be carefully estimated without blurring or over-sharpening of salient image structures, either of which can produce unwanted artifacts in the final exaggerated result.

%An alternative application with different criteria is image abstraction and pencil sketching \cite{L0smooth}.  Here the goal is to smooth out areas characterized by modest gradients while maintaining and enhancing salient sharp edges to create certain stylization effects.  As before though, inaccurate preservation of salient structures can be visually displeasing and/or completely misleading.  Likewise, as a final illustrative example, the removal of distracting small-scale textures, characterized by potentially high-contrast color transitions, can be viewed as a another specialized image smoothing problem \cite{RTV,RGF}, albeit one with very different requirements, i.e., either detail magnification \cite{WLS} or pencil sketching \cite{L0smooth} solutions will provably fail.

Unfortunately, no existing algorithm serves as an image smoothing panacea, and it is generally tedious to design independent solutions for each distinct application as has been traditionally done in the past.  We therefore investigate a novel unified framework that accommodates different image smoothing effects using only small, transparent modifications of a generic template.  In doing so we exploit the fact that the central step of any smoothing operator is the determination of which image structures to depress (image smoothing/flattening) and which parts to preserve or even enhance (edge-preservation).
%For example, at times we may wish to eliminate fine-scale high-contrast textures \cite{RTV}, while in others we may instead prefer to remove only low-amplitude details \cite{L0smooth}.
In this regard, our generic template is equipped with a convenient entry point for flexibly suppressing or enhancing application-dependent image structures.

To instantiate this proposal, we begin by structuring a new smoothing objective function with two key ingredients.  The first is a spatially-adaptive $L_p$ flattening criterion whereby the specific value of $p$ is varied across images in accordance with an application-specific guidance map.  Given that $p=2$ tends to smooth out edges, while $p \in (0,1]$ largely preserves them, this guidance map allows different image regions to receive different forms of regularization most appropriate for handling local structural conditions.
%For example, stair-casing artifacts produced by applying $p \in (0,1]$ to regions with small gradations, and conversely, blurred salient edges favored when $p=2$, can both be avoided.
This is dramatically different from many previous works whereby a single $L_p$ norm (or related) is applied across the entire image.  Importantly, the added flexibility afforded by the guidance map also allows for the seamless implementation of multiple different flattening effects.

Secondly, to explicitly fortify important edges that may be at least partially weakened by the flattening operator, we include a second criterion that minimizes the masked quadratic difference between edge maps computed from the original input image and the corresponding smoothed estimate respectively.  The masks are computed using a simple edge detection heuristic and can be manually modified further if desired.

Together with a standard data term to ensure structural similarity between input and output images, the combined objective function is non-convex with a combinatorial number of local minima.  Moreover, any costly attempt to even locally optimize the energy will only reflect the geometry of a single input image in isolation.  It would therefore be preferable to pool the information from multiple images loosely guided by the design criteria above, especially if this can be accomplished in a computationally efficient fashion.  Fortunately, recent deep neural network (DNN) approaches provide a natural candidate for addressing these issues.

It is crucial to emphasize up front, however, that our usage of deep networks is quite different from traditional applications to computer vision and graphics problems.  In the vast majority of existing cases, DNNs are trained to either predict external labels provided by human annotations (e.g. object detection, segmentation) or else to estimate the output of some computationally expensive algorithmic process of interest, such as an image smoothing filter \cite{xu2015,liu2016,fan2017generic,chen2017fast}.  For the latter, the idea is simply to construct a fully-labeled training set by running the original algorithmic process, and then learn a network to mimic its behavior at a fraction of the computational cost.  In these situations, the expectation is that the resultant network serves only as an approximation to the original process that generates the data.

In contrast, we consider an unsupervised, label-free setting, where the only input to our training platform is a corpus of images containing representative structures that we would ultimately like to smooth.  The loss function is then formed from the proposed objective function outlined above aggregated over all the training images. Moreover, under this circumstances, the deep network is treated as an optimizer or numerical solver to the objective function, instead of a commonly adopted regression tool in many other papers \cite{xu2015,liu2016,fan2017generic,chen2017fast}. At test time, a single image may be applied to the learned network, which will directly output the smoothed counterpart.

This unsupervised DNN-based process maintains a number of advantages over existing methods:  (i) Expensive labeled training data is not explicitly required, although weak forms of supervision can be introduced on an application-specific basis to improve performance, however which was not used for any of the results reported in this paper.
%For example, manually-annotated salient edges could be provided to improve formation of our energy function if desired.  Note however no such manual annotation was included for any of the results reported in this paper.  
(ii) The network weights reflect information from all images simultaneously, and are not restricted to simply predicting the (possibly flawed) outputs from a traditional solver that may at times converge to suboptimal solutions on individual images. (iii) When compared against classical smoothing algorithms that often require many expensive iterations to converge (if at all) for each new test image, once trained our network only requires a single feed-forward pass for evaluation which can be efficiently computed on both GPU and CPU.  (iv) Further improving test-time efficiency. Additional derived quantities (e.g., guidance maps) used to define our proposed network loss function during training are no longer needed.  With traditional methods this may not be the case.

% ***

%Deep learning has been successfully applied in directly learning the desired supervised target in an end-to-end manner for many computer vision and graphics tasks, e.g. object detection, segmentation, image super-resolution, reflection removal, etc. However, deep learning has been barely utilized as a solution to the optimization problem without ground truth labels for supervised training.
%
%In this paper, we treat deep learning as a numerical solver to optimize an objective function in an weakly-supervised way. The proposed objective function is implemented as a loss layer with back propagation which enables gradient descent in optimizing the deep neural network. In the learning stage, we train a deep network to iteratively minimize the objective function, and feed a new image through the network without the need of optimizing the objective function again in the evaluation stage.
%
%The deep learning solver makes a big difference from traditional optimization methods in mainly three sides, 1). The classical optimization process is usually computationally expensive and time consuming for many iterative minimizations. The deep learning solver is presented as a deep neural network, which requires only one feed forward pass for evaluation and is therefore usually very efficient. 2). An effective trivial solution to a sophisticated objective function is difficult to be resolved in many cases, while the restriction to a deep learning solution is very limited: as long as the objective function is differentiable to the optimized target, it can be trivially optimized by the deep network, which is very easy to implement. 3). Except for input image, extra inputs like guidance image in our proposed measures is no longer required in the evaluation stage, which is not the case for the traditional methods.

\input{fig-state_of_the_art.tex}

Broadly speaking, the contribution of this paper can be distilled to the following:
\begin{itemize}
\item We introduce a novel image smoothing objective function built upon the mixture of a spatially-adaptive $L_p$ flattening criterion and an edge-preserving regularizer. By minimizing the aggregate objective using a specialized deep network that simultaneously accounts for structure across a corpus of images, our approach is able to achieve state-of-the-art image smoothing effects in a variety of application domains.
\item We are able to implement multiple different image smoothing solutions within a single framework. The only variable responsible for modulating distinct, application-specific smoothing effects is a guidance edge map, which can be estimated using basic image processing principles and, if desired, further modified by the user.
\item During training our deep network requires only input images (no labels), or possibly weak supervision in the form of user annotations (note that for all experiments reported herein, we used no such user annotations).  Hence we are able to jointly learn from any sufficiently diverse corpus of images in a largely unsupervised manner unlike prior DNN approaches.  At test time, we obtain an efficient end-to-end mapping that takes a single image as input (no guidance map needed) and outputs the corresponding smoothed version with a computational footprint far below most traditional pipelines.
%In doing so we replace an image-specific learning process with.
%
% and possibly weak supervision from user-edits to the guidance map
\end{itemize}

%We propose a new deep learning based solution pipeline to the aforementioned image smoothing criterion. The optimization process is learned into the deep network which is represented as an end-to-end mapping for evaluation. The proposed solver runs much faster than most traditional image smoothing algorithms.

%*******************second version**********************
%Image smoothing is an essential tool to implement multiple different image processing and computer graphics applications. For example, edge preserving smoothing is required to generate some stylization effects like image abstraction, pencil sketching, \emph{etc}. By extracting the detail layer from the input and edge-preserving smoothing image, the subtle image details can be enhanced for better visualization. Specialized smoothing measure \cite{RTV} and framework \cite{RGF} are developed to remove the small-scale textures while maintaining the visually important image structures. More recently, the bokeh effects generated by the large aperture with professional lens has been approximated on the smart phones. Some famous app like Snapseed and smart phone producers like Huawei and Oppo have implemented similar functions to enable beautiful background blur effects. All the different applications demand specific and distinct design of the algorithm, for example, texture removal requires to eliminate the distractive repetitive small-scale structures where color transition may be even significant, however edge-preserving smoothing will maintain such edges.
%
%Various different smoothing effects can be implemented by minimizing the flattening criterion equipped with distinct $L_p$ norm. For example, $L_p$ norm (0<p<1) performs very well in achieving strong smoothing effects, but tends to create staircasing artifacts within moderate smooth regions by breaking them up into piecewise constant regions separated by spurious edges, while $L_p$ norm (p=2) is able to generate blurry images and wipe out the edges.
%
%To implement all the drastically different smoothing effects within a single framework, we propose a spatially variant $L_p$ norm flattening criterion, which applies $L_{0.5}$ and $L_2$ norm in distinct image regions in accordance to a user specified edge map. For the example of edge-preserving image smoothing, $L_{0.5}$ norm is utilized among the whole image except for the over-sharpened patchy regions, which are covered by $L_2$ norm to blur the spurious edges.
%
%As $L_{0.5}$ norm is employed, the smooth image becomes sharp, and the edges with conspicuous color transition are easily maintained well. By minimizing the flattening criterion, the nearby pixels with similar colors tends to be put even closer. Some slender edges whose two sides share similar color values tend to be over smoothed, but they still could be semantically important. To overcome the challenges, we present an edge-preserving criterion to explicitly highlight the desired valuable structures guided by the same edge map utilized in the flattening criterion.
%
%To transform between different smoothing applications within the same framework, we only need to adjust the feeded edge map which indicates various smoothing effects in distinct regions.
%
%Instead of exploiting traditional numerical solver to optimize the objective function, in this paper, we propose to employ an efficient fully-convolutional deep neural network which learns to minimize the proposed criterions. Note the benefits of our deep learning based solver lies in three aspects. \emph{(a)}, the deep network is learned as an end-to-end mapping which characterizes the smoothing effects. It requires only the input image for evaluation since the guided edge map is incorporated into the criterions for only training. \emph{(b)}, our deep learning based solver runs much faster than the other optimization based smoothing strategies, as only one forward pass is needed for testing instead of multiple iterations in traditional methods. \emph{(c)}, deep learning provides a new pathway to optimize the objective functions which are too complex to find an efficient and effective traditional solver. The details of optimization process is represented in the deep network.
%
%All in all, the contribution of this paper lies as follows,
%\begin{itemize}
%\item We introduce a new image smoothing measure, built on the mixture of a spatially adaptive $L_p$ norm flattening criterion and an edge-preserving criterion guided by the same edge map. By minimizing the proposed criterions, our algorithm is able to achieve state-of-the-art various different image smoothing effects.
%\item We are the first to implement multiple different image smoothing effects within a single framework, such as edge-preserving smoothing, texture removal, background blur out of saliency, \emph{etc}. The only variable responsible for the distinct smoothing effects is the edge map, which can be detected or even user designed.
%\item We propose a new deep learning based solution pipeline to the above image smoothing criterion. The optimization process is learned into the deep network which is represented as an end-to-end mapping for evaluation. The proposed solver is very efficient and doesn't require the guided edge map in the test stage.
%\end{itemize}
%*******************second version**********************




%*******************first version**********************
%Various degrees of details and structures are filled in natural images. To perform a better manipulation and understanding of the scene, it is crucial to extract the sparse salient structures and diminish the insignificant details in accordance with human visual perception, which is exactly the goal of edge-preserving image smoothing. The generality and effectiveness of this technique is exemplified in many image processing and computer graphics tasks, like edge extraction, image stylization, pencil sketching, detail enhancement, \emph{etc}.


%Edge aware image smoothing can be achieved by filtering based strategies \cite{anisotropic,BLF98,paris2006fast,weiss2006fast,DT}, which generally calculates the smooth image as a weighted average of the input image. As the above methods are highly restricted to the pixels in the local neighbourhood, the optimization-based approaches \cite{WLS,L0smooth,RTV,FGS,L1smooth} has attracted considerable attention in the last decade, which iteratively seeks a global optimal solution to the objective function which contains a prior flattening term in the sparsity-inducing norm. However, as observed in \cite{L0smooth}, while the smoothing weight becomes larger or the norm becomes smaller, the smooth images tend to be over sharpened and some meaningful edges are diminished by mistake. Moreover, the iterative optimization process is usually complex and time-consuming. Designing a simple and fast solver to the objective function is not easy, either.
%
%To tackle the aforementioned challenges, we propose the hybrid $L_p$/$L_2$ norm based flattening criterion\footnote{In this paper, the constraint ($p < 1$) is defined for $L_p$ norm.}, which not only seeks high-quality smoothness effects with $L_p$ norm, but also overcomes the side effects induced by $L_p$ norm by exploiting $L_2$ norm among the over-sharpened areas. To keep the over-smoothed edges while strong smoothing effect is applied, we present an edge-preserving criterion for explicitly emphasizing these detected thin yet important edges. Since the image structure is maintained well, each separated region becomes even more smoother, and its color is less mixed from the color of other regions.
%
%Unlike previous optimization based smoothing papers, we don't seek an explicit solution to optimize the energy function, but hide the optimization process in an end-to-end mapping learned as a deep neural network, and request only one forward pass given a new natural image, instead of multiple iterations in traditional methods. This is significantly faster than most filtering or optimization based smoothing methods. It treats the detailed solution to the energy function as a black box implemented in the deep neural network. The burden for developing a simple and fast solver is eased from the researchers.
%
%*******************first version********************** 
